Small batch deep reinforcement learning

In value-based deep reinforcement learning with replay memories, the batch size parameter specifies how many transitions to sample for each gradient update. Although critical to the learning process, this value is typically not adjusted when proposing new algorithms. In this work we present a broad empirical study that suggests {\em reducing} the batch size can result in a number of significant performance gains; this is surprising, as the general tendency when training neural networks is towards larger batch sizes for improved performance. We complement our experimental findings with a set of empirical analyses towards better understanding this phenomenon.

==> sections/broaderImpact.tex <==
\paragraph{Broader impact} Although the work presented here 
is mostly of an academic nature, it aids in the development of more capable autonomous agents. While our
contributions do not directly contribute to any negative
societal impacts, we urge the community to consider
these when building on our research

==> sections/takeaways.tex <==
\section{In summary}
Having presented the empirical advantages of reduced batch sizes (\autoref{sec:varyingbatchsize_effects}) and an extensive analysis of its possible causes (\autoref{sec:potential_causes}), we summarize the main takeaways below:
\begin{enumerate}
    \item When training online value-based agents, smaller batch sizes are better.
    \item Smaller batch sizes avoid performance plateaus when extending training times.
    \item When exploring multi-step returns, smaller batch sizes are preferable.
    \item Smaller batch sizes can produce a ``natural'' form of exploration.
\end{enumerate}
